POLAR: Preference Optimization and Learning Algorithms for Robotics

Parameter tuning for robotic systems is a time-consuming and challenging task that often relies on domain expertise of the human operator. Moreover, existing learning methods are not well suited for parameter tuning for many reasons including: the absence of a clear numerical metric for `good robotic behavior'; limited data due to the reliance on real-world experimental data; and the large search space of parameter combinations. In this work, we present an open-source MATLAB Preference Optimization and Learning Algorithms for Robotics toolbox (POLAR) for systematically exploring high-dimensional parameter spaces using human-in-the-loop preference-based learning. This aim of this toolbox is to systematically and efficiently accomplish one of two objectives: 1) to optimize robotic behaviors for human operator preference; 2) to learn the operator's underlying preference landscape to better understand the relationship between adjustable parameters and operator preference. The POLAR toolbox achieves these objectives using only subjective feedback mechanisms (pairwise preferences, coactive feedback, and ordinal labels) to infer a Bayesian posterior over the underlying reward function dictating the user's preferences. We demonstrate the performance of the toolbox in simulation and present various applications of human-in-the-loop preference-based learning.

==> Sections/char_experiments.tex <==
\section{Experimental Results towards Characterizing Exoskeleton User Preference Landscapes}
\label{Sec: exp_char}

In this section, we present and discuss the experimental results of applying the ROIAL algorithm towards learning a four-dimensional preference landscape for 3 non-disabled exoskeleton subjects. First we will discuss the details of the experimental setup, followed by the experimental results.

\subsection{Experimental Setup}
The ROIAL algorithm was deployed\footnote{Kernel: squared exponential with lengthscales = $[0.02,5,1,1.2]$, signal variance = 1, noise variance = 1e-5, $c_p$ = 0.0015, $c_o = 0.1$, $\lambda = 0.45$ \label{footnote: hyper_roial}} towards preference characterization over a four-dimensional action space for a total of three non-disabled subjects using the same gait library as used in the LineCoSparV1 experiments, outlined in Table \ref{table: linecospar}, but with fixed values for step width and step height. Thus, each action constructed as: $\act := [a_1, a_2, a_5, a_6] \in \R^{11 \times 7 \times 5 \times 5}$, leading to an action space with cardinality $|\actions| = 1925$. More concretely, $\actions$ was defined over four gait parameters: step length (SL), step duration (SD), pelvis pitch (PP), and pelvis roll (PR). Note that the action space was purposefully constructed to have fewer actions than that of the LineCoSpar experiments since active learning requires more information than regret minimization. 

The experimental procedure was the same as the CoSpar and LineCoSpar experiments, except that the user was queried for a pairwise preference and an ordinal label. Coactive feedback was not included as a feedback mechanism for these experiments since providing the algorithm with more information about user preferred actions could bias the exploration towards actions with lower utilities. However, future experiments could benefit from the inclusion of coactive feedback since it provides more information about the underlying utility function. Instead, the experiments queried the user for an ordinal label belonging to one of four ordinal categories. These four categories were described to the users as:
\begin{enumerate}
    \item \textbf{Very Bad} ($\mathbf{O}_1$): User feels unsafe or uncomfortable to the point that the user never wants to repeat the gait.
    \item \textbf{Bad} ($\mathbf{O}_2$): User dislikes the gait but does not feel unsafe or uncomfortable.
    \item \textbf{Neutral} ($\mathbf{O}_3$): User neither dislikes nor likes the gait and would be willing to try the gait again.
    \item \textbf{Good} ($\mathbf{O}_4$): User likes the gait and would be willing to continue walking with it for a long period of time. 
\end{enumerate} 
While including additional ordinal categories could increase the information gained from each query, it also increases the cognitive burden for the users, thus reducing reliability.

\vspace{-1em}
\subsection{Experimental Results}
Since the ROIAL algorithm provides reliable information across the entire ROI, we can gain insights from observing each subject's preference landscape, shown in Figure \ref{fig: roialpost}. Mainly, we can observe regions of agreement and disagreement among the subjects. For example, all subjects strongly dislike gaits at the lower bound of PP and lower bound of PR. However, all subjects disagree in their utility landscapes across SL and SD. This type of insight could not be derived from direct gait optimization, which mostly obtains information near the optimum. Unfortunately, making conclusive claims about why subjects prefer certain gaits over others requires data from more subjects. However, these experimental results validate that the ROIAL algorithm is a sample-efficient method of obtaining preference landscapes, while also avoiding gaits that make the user feel uncomfortable or unsafe. 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/ROIAL/ROIAL_landscapes.png}
    \caption{This figure illustrates the four-dimensional preference landscapes obtained using the ROIAL algorithm for each non-disabled subject, with each plot showing the posterior mean plotted over two dimensions and averaged over the remaining two. The averaged posterior means were normalized by subject, with each subject shown in each rows, and each two-dimensional projection shown in each column. The dimensions are abbreviated: Step Length (SL), Step Cadence (SC), Pelvis Roll (PR), and Pelvis Pitch (PP). These preference landscapes illustrate regions of agreement and disagreement across subjects. Two specific gaits are illustrated using gait tiles at the bottom: the left illustrates a gait with values of PR and SC that were liked across subjects; the right illustrates a gait with values of PR and PP that were disliked across subjects. It can also be seen that the distribution of sampled gaits, shown by the black circles, was more uniform across the action space compared to the Preference Optimization experiments.}
    \label{fig: roialpost}
\end{figure*}

\newsubsec{Evaluation of Preference Accuracy}
At the conclusion of the 30 iterations, the subjects unknowingly entered a \textit{validation phase} which consisted of 10 additional iterations. The purpose of this validation phase was to collect true user ordinal labels on 10 new exoskeleton gaits, and compare this true user feedback with the ordinal labels predicted by the final posterior mean as a method of evaluating the accuracy of the learned preference landscape. These additional 10 gaits are termed ``validation actions'' and they were selected so that at least two samples were predicted to belong to $\mathbf{O}_2, \mathbf{O}_3$, and $\mathbf{O}_4$, with the remaining four validation actions sampled at random. Actions predicted to belong in $\mathbf{O}_1$ were excluded because they are likely to make the user feel uncomfortable or unsafe. Actions sampled during the training phase (initial 30 iterations) were also explicitly excluded from the validation trials.

Figure \ref{fig:exo_confusion} depicts the results of the validation phase for all three subjects. These results show a reliable correlation between the predicted categories and the users' reported ordinal labels, in which the majority of the predicted ordinal labels are within one category of the true ordinal labels. Since less than $2\%$ of the action space was explored during the experiment, we expect that the prediction accuracy would increase with additional exoskeleton trials.

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.36\textwidth]{Figures/ROIAL/exo_confusion_matrix_column_boxed.png}
    \vspace{-1.5mm}
      \caption{Confusion matrix of the validation phase results for all three subjects. The first column is grey because actions in the ROA ($\mathbf{O}_1$) were purposefully avoided to prevent subject discomfort. Percentages are normalized across columns. Parentheses show the numbers of gait trials in each case.}
  \label{fig:exo_confusion}
\vspace{-6.32mm}
\end{figure}


==> Sections/dim-reduction.tex <==
\section{Dimensionality Reduction Techniques for High-Dimensional Action Spaces}
\label{Sec: dimreduction}

\subsection{Dimensionality Reduction for Regret Minimization}
To reduce this computational complexity of our framework towards regret minimization, we use an approach inspired by \cite{kirschner2019adaptive}. The full preference optimization algorithm with our proposed dimensionality reduction method was originally named LineCoSpar \cite{tucker2020human} and is outlined in Alg. \ref{alg: linecospar}.

The main idea of our approach is to construct $\sub := \randline \cup \vis$ to be the union of actions along a random line $\randline \subset \actions$ and the previously sampled actions $\vis$. The random line $\randline$ is generated such that it intersects the action maximizing the posterior mean $\hat{a}^*$ from the most recently obtained user data. The method of Thompson sampling is then identical as before, except instead of drawing samples over $\mathcal{N}(\mu_{\actions},\Sigma_{\actions})$, samples are drawn over $\mathcal{N}(\mu_{\sub},\Sigma_{\sub})$. Consequently, possible sampled actions are only the actions that lie in $\sub$, however \cite{kirschner2019adaptive} found that this approach still yielded state-of-the-art performance with significantly reduced computational complexity. 

Note that to update $\hat{a}^*$ after executing the actions obtained through Thompson sampling, the posterior must be approximated again using the new user feedback. However, this second posterior update is only inferred over the set of all executed actions $\vis$ to yield the posterior distribution $\N(\mu_{\vis},\Sigma_{\vis})$. The believed optimal action is then calculated as $\hat{a}^* = \argmax_{a \in \vis} \mu_{\vis}(a)$.

Thus, this method of dimensionality reduction for Thompson sampling requires updating the posterior twice in each iteration: once at the beginning of the iteration to compute $\mathcal{N}(\mu_{\sub}, \Sigma_{\sub})$, and once at the end of the iteration to compute $\mathcal{N}(\mu_{\vis}, \Sigma_{\vis})$ that is then used to update $\hat{a}^*$. Even though this method requires updating the posterior twice, both of these computations are significantly cheaper than computing the posterior over the entire action space.


\subsection{Dimensionality Reduction for Active Learning}
The dimensionality reduction approach for the active learning setting is similar to that of the regret minimization setting in that it reduces the computational complexity by only inferring the Bayesian posterior over a subset of actions $\sub$. However, since the objective is to characterize the entire utility function within the ROI, the composition of $\sub$ is different. For active learning, $\sub$ is selected as a set of $R$ random actions combined with the previously sampled actions: $\sub := \act_{\text{rand}} \cup \vis$ with $\act_{\text{rand}} = \{ a_{\text{rand}}^{(i)} \in \actions \mid i = 1,\dots,R\}$. A larger $R$ results in a better approximation of $P(\utilvec,\prefdata,\coacdata,\orddata)$ which important for determining the information gain as explained in Section. \ref{Sec: sampling}. However, a larger $R$ also leads to the original problem of computational complexity. Thus, $R$ becomes a user-determined hyperparameter of the learning depending on the size of the action space. In our experiments, $R$ was selected to be 500 for an action space with 1,750 actions. \red{Figure \ref{fig: subsetsize} demonstrates the tradeoff between $R$ and the speed of learning. discuss results of figure once it's made. }

As also mentioned in Section \ref{Sec: sampling}, only maximizing the information gain for one action at a time significantly reduces the computational complexity of the proposed active learning framework. For this reason, we recommend only sampling one action at a time ($n = 1$) when doing preference characterization with information gain. This dimensionality reduction approach for Information Gain is outlined in Alg. \ref{alg: roial}.



%  \begin{figure}[tb]
%     \centering
%     \includegraphics[width=\linewidth]{example-image-a}
%     \caption{Effect of $R$ on Active Learning}
%     \label{fig: subsetsize}
% \end{figure}


==> Sections/discussion.tex <==
\section{Discussion}
\label{Sec: discussion}

\section{Preference optimization vs. characterization}

As expected, the choice between preference optimization and preference characterization largely influences the obtained experimental results. Since preference optimization is aimed at locating the gait parameters that optimize the exoskeleton user's preferences as quickly as possible, the algorithm prioritizes exploitation and consequently does not provide an accurate understanding of the entire utility function. Alternatively, since the goal of preference characterization is to learn the entire underlying utility function, it does so but it necessarily requires either more informative feedback achieved through the use of ordinal feedback, or it requires more experimental iterations.

\section{Extracting information from obtained preference landscapes}

==> Transactions-Bibliography/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

